Approximability of Discriminators Implies Diversity in GANs

While Generative Adversarial Networks (GANs) have empirically produced impressive results on learning complex real-world distributions, recent works have shown that they suffer from lack of diversity or mode collapse. The theoretical work of Arora et al. suggests a dilemma about GANs' statistical properties: powerful discriminators cause overfitting, whereas weak discriminators cannot detect mode collapse. By contrast, we show in this paper that GANs can in principle learn distributions in Wasserstein distance (or KL-divergence in many cases) with polynomial sample complexity, if the discriminator class has strong distinguishing power against the particular generator class (instead of against all possible generators). For various generator classes such as mixture of Gaussians, exponential families, and invertible and injective neural networks generators, we design corresponding discriminators (which are often neural nets of specific architectures) such that the Integral Probability Metric (IPM) induced by the discriminators can provably approximate the Wasserstein distance and/or KL-divergence. This implies that if the training is successful, then the learned distribution is close to the true distribution in Wasserstein distance or KL divergence, and thus cannot drop modes. Our preliminary experiments show that on synthetic datasets the test IPM is well correlated with KL divergence or the Wasserstein distance, indicating that the lack of diversity in GANs may be caused by the sub-optimality in optimization instead of statistical inefficiency.

==> cleantex-new/experiment-full.tex <==
\section{Simulations}\label{sec:exp}
We perform synthetic WGAN experiments with invertible neural net
generator (cf. Section~\ref{section:invertible-generator}) and
discriminator designed with restricted approximability
(Lemma~\ref{lemma:logp-neural-network}). Our main goal is to demonstrate that the empirical IPM $W_{\cF}(p,q)$ is well correlated with the KL-divergence between $p$ and $q$ on synthetic data, in for various pairs of $p$ and $q$ (The true distribution $p$ is generated randomly from a ground-truth neural net, and the distribution $q$ is learned using various algorithms or perturbed version of $p$.) 

We recall that the main technical contribution of the paper is on the injective neural networks where the data distribution has low-dimensional supports (Section~\ref{s:additive}). However, since the guarantees are in the Wasserstein distance that is not efficiently and provably computable, we don't have experiments that directly justify the theory there. %We remark that in the authors' opinion, 
%Principled evaluation of the diversity of GANs is a major open question in the field and is beyond the scope of this paper. 

%\Tnote{added paragraph above}
\subsection{Setup}
\paragraph{Data}
The data is generated from a ground-truth invertible
neural net generators (cf. Section~\ref{section:invertible-generator}), i.e. $X=G_\theta(Z)$, where
$G_\theta:\R^d\to\R^d$ is a $\ell$-layer layer-wise invertible
feedforward net, and $Z$ is a spherical Gaussian. We use the Leaky ReLU with negative slope 0.5 as the
activation function $\sigma$, whose derivative and inverse can be very
efficiently computed. The weight matrices of the layers are set to be
well-conditioned with singular values in between $0.5$ to $2$.

\sloppy We choose the discriminator architecture according to the
design with restricted approximability guarantee
(Lemma~\ref{lemma:logp-neural-network}, equation~\eqref{eqn:F-1}
and~\eqref{eqn:F-2}). As $\log\sigma^{-1'}$ is a piecewise constant
function that are not differentiable, we instead model it as a
trainable one-hidden-layer neural network that maps reals to reals. We
add constraints on all the parameters in accordance with
Assumption~\ref{assumption:invertible-generator}.

\paragraph{Training}
To train the generator and discriminator networks,  we generate stochastic batches (with batch
size 64) from both the ground-truth generator and the trained
generator, and solve the min-max problem in the Wasserstein GAN
formulation. We perform 10 updates of the discriminator in between each
generator step, with various regularization methods for discriminator
training (specified later). We use the RMSProp
optimizer~\cite{TielemanHi12} as our update rule. 

\paragraph{Evaluation metric}
We evaluate the following metrics between the true and learned
generator.
\begin{enumerate}[(1)]
\item The KL divergence. As the density of our invertible neural net
  generator can be analytically computed, we can compute their KL
  divergence from empirical averages of the difference of the log densities: 
  \begin{equation*}
    \what{\dkl}(p^\star,p) = \E_{X\sim\what{p^\star}^n}[\log
    p^\star(X)-\log p(X)],
  \end{equation*}
  where $p^\star$ and $p$ are the densities of the true generator and
  the learned generator. We regard the KL divergence as the
  ``correct'' and rather strong criterion for distributional
  closedness.
\item The training loss (IPM $W_{\cF}$ train). This is the
  (unregularized) GAN loss during training. Note: as typically in the training of GANs, we balance carefully the number of steps for discriminator and generators, the training IPM is potentially very away from the true $W_{\cF}$ (which requires sufficient training of the discriminators).
\item The neural net IPM ($W_{\cF}$ eval). We report once in a
  while a separately optimized WGAN loss in which the learned
  generator is held fixed and the discriminator is trained from
  scratch to optimality. Unlike the training loss, here the
  discriminator is trained in norm balls but with no other
  regularization. By doing this, we are finding $f\in\cF$ that
  maximizes the contrast and we regard the $f$ found by stochastic
  optimization an approximate maximizer, and the loss obtained an approximation of $W_{\cF}$.
\end{enumerate}

Our theory shows that for our choice of $\mc{G}$ and
$\mc{F}$, WGAN is able to learn the true generator in KL divergence,
and the $\cF$-IPM (in evaluation instead of training) should be indicative of the KL
divergence. We test this hypothesis in the following experiments.

\vspace{0.1cm}

\subsection{Convergence of generators in KL divergence}
\label{section:experiment-convergence}
In our first experiment, $G$ is a two-layer net in $d=10$
dimensions. Though the generator is only a shallow neural net,
the presence of the nonlinearity makes the estimation problem
non-trivial. We train a discriminator with the architecture specified
in Lemma~\ref{lemma:logp-neural-network}),
using either Vanilla WGAN (clamping the weight into norm balls) or
WGAN-GP~\cite{GulrajaniAhArDuCo17} (adding a gradient penalty). We fix
a same ground-truth generator and run each method from
6 different random initializations. Results are plotted in
Figure~\ref{figure:conjoined}.

Our main findings are two-fold:
\begin{enumerate}[(1)]
\item WGAN training with discriminator design of restricted
  approximability is able to learn the true distribution in KL
  divergence. Indeed, the KL divergence starts at around 10 - 30 and
  the best run gets to KL lower than 1. As KL is a rather strong
  metric between distributions, this is strong evidence that GANs are
  finding the true distribution and mode collapse is not happening.
\item The
  $W_{\cF}$ (eval) and the KL divergence are highly correlated with each
  other, both along each training run and across different runs. In
  particular, adding gradient penalty improves the optimiztaion significantly
  (which we see in the KL curve), and this improvement is also reflected
  by the $W_{\cF}$ curve. Therefore the quantity $W_{\cF}$ can serve
  as a good metric for monitoring convergence and is at least much
  better than the training loss curve.
\end{enumerate}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/figure-arxiv-1.png}
  \caption{\small Learning an invertible neural net generator on
    synthetic data.  The x-axis in all the graphs indicates the number
    of steps. The left-most figure shows the KL-divergence between the
    true distribution $p$ and learned distribution $q$ at different
    steps of training, the middle the estimated IPM (evaluation)
    between $p$ and $q$, and the right one the training loss. We see
    that the estimated IPM in evaluation correlates well with the
    KL-divergence. Moving average is applied to all curves. }
  \label{figure:conjoined}
\end{figure}

To test the necessity of the specific form of the
discriminator we designed, we re-do the same experiment with vanilla
fully-connected discriminator nets. Results (in
Appendix~\ref{appendix:experiment-vanilla}) show that IPM with vanilla
discriminators also correlate well with the KL-divergence. This is not
surprising from a theoretical point of view because a standard
fully-connected discriminator net (with some over-parameterization) is
likely to be able to approximate the log density of the generator
distributions (which is essentially the only requirement of
Lemma~\ref{thm:logp}.)

For this synthetic case, we can see that the inferior performance in KL of the WGAN-Vanilla algorithm doesn't come from the statistical properties of GANs, but rather the inferior training performance in terms of the convergence of the IPM. We conjecture similar phenomenon occurs in training GANs with real-life data as well. 


\subsection{Perturbed generators}
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\columnwidth]{figures/figure-arxiv-3.png}
  \caption{Scatter plot of KL divergence and neural net IPM on
    perturbed generator pairs. Correlation between
    $\log(\dkl(p\|q)+\dkl(q\|p))$ and 
    $\log\df$ is 0.7315. Dashed line is
    $\df(p,q)=100(\dkl(p\|q)+\dkl(q\|p))$.}
  \label{figure:correlation}
\end{figure}

In this section, we remove the effect of the optimization and directly
test the correlation between $p$ and its perturbations. 
We compare the KL
divergence and neural net IPM on pairs of {\it perturbed
  generators}.  In each instance, we generate a pair of generators
$(G,G')$ (with the same architecture as above), where $G'$ is a
perturbation of $G$ by adding small Gaussian noise.
We compute the KL divergence
and the neural net IPM between $G$ and $G'$. To denoise the
unstable training process for computing the neural net IPM, we
optimize the discriminator from 5 random initializations and pick the
largest value as the output.

As is shown in Figure~\ref{figure:correlation}, there is a clear
positive correlation between the (symmetric) KL divergence and the
neural net IPM.
In particular, majority of the points fall around
the line $\df=100\dkl$, which is consistent with our theory that the
neural net distance scales linearly in the KL divergence.
Note that there are a
few points with outlyingly large KL. This happens mostly due to the
perturbation being accidentally too large so that the weight
matrices become poorly conditioned -- in view of our theory, they fall
out of the good constraint set as defined in
Assumption~\ref{assumption:invertible-generator}.




==> cleantex-new/experiment.tex <==
\section{Experiments}
We perform synthetic WGAN experiments with invertible neural net
generator (cf. Section~\ref{section:invertible-generator}) and
conjoined discriminator design
(Lemma~\ref{lemma:logp-neural-network}). We focus on comparing
the KL divergence and the neural net distance, either during
training or between specifically chosen pairs of generators. Details
on the experimental setup are described in
Appendix~\ref{appendix:experiment}.

\vspace{0.1cm}

\noindent{\bf Convergence of generators in KL divergence.}
In our first experiment, $G$ is a two-layer net in $d=10$
dimensions. Though a shallow generaotr, presence of the nonlinearity
makes the estimation problem non-trivial. 
We find that WGAN training with conjoined discriminator design
approaches the true distribution in the KL divergence
(Figure~\ref{figure:figure} left and middle). Along training, the
neural net distance, though very noisy (due to the difficult
optimization landscape of GANs), shows positive correlation with
the KL divergence after smoothing. This observation is consistent with
our theory, which says that the KL divergence and the neural net
distance are bounded by each other.


\vspace{0.1cm}

\noindent{\bf Perturbed generators.}
To further get rid of the optimization difficulties, we compare the KL
divergence and neural net distance on pairs of {\it perturbed
  generators}.  In each instance, we generate a pair of generators
$(G,G')$ (with the same architecture as above), where $G'$ is a
perturbation of $G$ by adding small Gaussian noise.
We compute the KL divergence
and the neural net distance between $G$ and $G'$. To denoise the
unstable training process for computing the neural net distance, we
optimize the discriminator from 5 random initializations and pick the
largest value as the output.

As is shown in Figure~\ref{figure:figure} right, there is a clear
positive correlation between the (symmetric) KL divergence and the
neural net distance. In particular, majority of the points fall around
the line $\df=100\dkl$, which is consistent with our theory that the
neural net distance scales linearly in the KL divergence. Note that a
few points have much larger KL than should be on the line, which is
because the perturbation there is too large so that the weight
matrices become poorly conditioned -- in view of our theory, they fall
out of the good constraint set as defined in
Assumption~\ref{assumption:invertible-generator}.

\begin{figure}
  \centering
  \includegraphics[width=0.8\columnwidth]{Figures/figure-3.png}
  \caption{\small Experiments on the invertible neural net generator
    and conjoined discriminator design.  Left and middle: Convergence
    of GAN training in KL divergence and neural net distance (with
    moving average smoothing at level 0.9). Observe the correlation
    between the two distances (e.g. blue, red for good performance,
    orange and cyan for poor performance). Note that the yellow curve
    blows up on both (KL too large to show).
    Right: Scatter plot of KL divergence and neural net distance on
    perturbed generator pairs. Dashed line is $\df=100\dkl$.}
  \label{figure:figure}
\end{figure}


==> cleantex-new/tools.tex <==


